Minimum Overhead Beamforming and Resource Allocation in D2D Edge Networks

Device-to-device (D2D) communications is expected to be a critical enabler of distributed computing in edge networks at scale. A key challenge in providing this capability is the requirement for judicious management of the heterogeneous communication and computation resources that exist at the edge to meet processing needs. In this paper, we develop an optimization methodology that considers the network topology jointly with device and network resource allocation to minimize total D2D overhead, which we quantify in terms of time and energy required for task processing. Variables in our model include task assignment, CPU allocation, subchannel selection, and beamforming design for multiple-input multiple-output (MIMO) wireless devices. We propose two methods to solve the resulting non-convex mixed integer program: semi-exhaustive search optimization, which represents a "best-effort" at obtaining the optimal solution, and efficient alternate optimization, which is more computationally efficient. As a component of these two methods, we develop a novel coordinated beamforming algorithm which we show obtains the optimal beamformer for a common receiver characteristic. Through numerical experiments, we find that our methodology yields substantial improvements in network overhead compared with local computation and partially optimized methods, which validates our joint optimization approach. Further, we find that the efficient alternate optimization scales well with the number of nodes, and thus can be a practical solution for D2D computing in large networks.

==> analysis.tex <==
\section{Algorithm Analysis}
\label{sec:analysis}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Optimality}
%\label{ssec:nro}

%We propose two different algorithms to solve for $a_{k,k'}$ and $b_{n,i}$ with ${\bf{f}}_{k}$, ${\bf{z}}_{k'}$ and $P_{k}$ fixed.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Convergence}
%\label{ssec:greedy}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Computational complexity}
%\label{ssec:greedy}




%%
$\\$

==> formulation.tex <==
\section{Optimization Formulation}
\label{sec:formulation}

In this subsection,
we formulate the problem of jointly optimizing 
task assignment $\{a_{k,k'}\}$, computation resource allocation $\{\delta_{k,k'}\}$, subchannel allocation 
$\{b_{k,i}\}$, and MIMO signal design involving 
transmit powers $\{P_k\}$, transmit beamformers $\{{\bf{f}}_{k}\}$, and receive combiners $\{{\bf{z}}_{k',i}\}$, which will lead to minimum total network demand ${\mathcal{C}}_{\rm{total}}$, given in \eqref{eq:obj:Utotal}. 
Therefore, we formulate the following optimization problem:
\begin{align}
& \text{minimize} & & \mathcal{C}_{\rm{total}}
\label{eq:obj:optCtotal} \\
& \text{subject to}
& &  \sum\nolimits_{k' =1}^K a_{k,k'} = 1 \;\; \forall k, 
\label{eq:con:a1} \\
& & & a_{k,k'} \in \{0,1\} \;\; \forall k,k',
\label{eq:con:a2} 
%\nonumber 
\\
& & & 
\sum\nolimits^S_{i=1} b_{k,i} = \left\{ {\begin{array}{*{20}{l}}
1 \quad \forall k \;\;
{\rm{with}} \;\; a_{k,k} = 0
\\
0 \quad \forall k \;\;
{\rm{with}} \;\; a_{k,k} = 1
\end{array}} \right.
\label{eq:con:b1}
\\
& & & \sum\nolimits_{k \in \mathcal{A}_{k'}} b_{k,i} \le 1 \;\; \forall k',i,
\label{eq:con:b2}
\\
& & & b_{k,i} \in \{0,1\} \;\; \forall k,i,
\label{eq:con:b3} 
%\nonumber 
\\
& & & R_{k,k'} \; \mbox{defined in (\ref{eq:rate})},
%\;\; \forall k,k' 
\label{eq:con:R} 
%\\
%& & & \quad \quad \quad 
%\mbox{with} \; a_{k,k}=0,
%\; \mbox{and} 
%\;
%\nonumber 
\\
& & & || {\bf{f}}_{k} ||_2 = 1 \;\; \forall k, \;\; || {\bf{z}}_{k',i} ||_2 = 1 \;\; \forall k',i, \label{eq:con:fz} \\
& & & 0 \leq P_{k} \leq P \;\; \forall k, 
\label{eq:con:P1} \\
%& & & P_{k} = 0 \;\; \forall k \;\; \mbox{with} \;\; b_{k,i} = 0,
%\label{eq:con:P2} 
%\nonumber 
%\\
& & &  F_{k,k'} \ge 0 \;\; \forall k,k', 
%\nonumber 
\label{eq:con:F1} 
\\
& & & F_{k,k'} = 0 \;\; \forall k,k' \;\; \mbox{with} \;\; a_{k,k'} = 0,
\label{eq:con:F2} 
\\
& & & \sum\nolimits^K_{k =1} F_{k,k'} \le {\mathrm{F}}_{k'} \;\; \forall k',
\label{eq:con:F3} 
\\ 
& \text{variables} 
& & \{{\bf{f}}_{k}\}, \{{\bf{z}}_{k',i}\}, \{P_{k}\}, \{F_{k,k'}\}, \{a_{k,k'}\}, \{b_{k,i}\} \nonumber
\end{align}
%
Constraint \eqref{eq:con:a1}-\eqref{eq:con:a2}, \eqref{eq:con:b1}-\eqref{eq:con:b3}, and \eqref{eq:con:F1}-\eqref{eq:con:F3} account for  task assignment, subchannel allocation and CPU allocation, which are described in Sec \ref{ssec:TaskAssignment}. 
In addition, Constraint \eqref{eq:con:fz}-\eqref{eq:con:P1} indicate the constraints for the MIMO signal variables, where in \eqref{eq:con:P1} we impose an transmission power budget $P$ on individual node.

Assuming all nodes have $N$ transmit and receive antennas, i.e., $N = N_{k}^{\text{tx}} = N_{k}^{\text{rx}}$ for all $k$, 
the optimization \eqref{eq:obj:optCtotal}-\eqref{eq:con:F3} is a mixed integer program (MIP) with $K(N+NS+1+K)$ non-integer variables from  
$\{{\bf{f}}_{k}\}$, $\{{\bf{z}}_{k',i}\}$, $\{P_{k}\}$, and $\{F_{k,k'}\}$,
and $K(K + S)$ integer variables from $\{a_{k,k'}\}$ and $\{b_{k,i}\}$. 
Also, since ${\mathcal C}_{\rm comm}$ as a function of $P_k$ has the form $x / \log(1+x)$, which is non-convex, the problem is a non-convex MIP.
Existing solvers for non-convex MIPs do not scale well with the number of variables \cite{burer2012non}, and even with $K=20$ nodes, $S=5$ subchannels, and $N=10$ antennas, our problem has more than 2000 variables.
One of the challenges is developing an effective algorithm to solve this problem. 
To this end, we propose two algorithms which are addressed in Sec. \ref{sec:algorithm}.

==> related.tex <==
\section{Related Work}
\label{sec:related}
